Translating Videos to Natural Language Using Deep Recurrent Neural Networks

Solving the visual symbol grounding problem has long been a goal of artificial intelligence. The field appears to be advancing closer to this goal with recent breakthroughs in deep learning for natural language grounding in static images. In this paper, we propose to translate videos directly to sentences using a unified deep neural network with both convolutional and recurrent structure. Described video datasets are scarce, and most existing methods have been applied to toy domains with a small vocabulary of possible words. By transferring knowledge from 1.2M+ images with category labels and 100,000+ images with captions, our method is able to create sentence descriptions of open-domain videos with large vocabularies. We compare our approach with recent work using language generation metrics, subject, verb, and object prediction accuracy, and a human evaluation.

==> future_work.tex <==

Future Work
1. An encoder-decoder model, instead of a decoder only model. Will automatically
identify a suitable pooling over frames of features.
2. Beam search
3. End-to-End trainable model similar to image description.

# below are tricks not necessary to mention.
4. Using features other than fc7 (fc6?)
5. Input image only in the first time step (for the decoder model). Google says
it prevents overfitting and performed better.
6. Have a single LSTM layer.


==> model.tex <==
\section{Approach}
\label{sec:approach}

\begin{figure}[t]
\begin{center}
   \includegraphics[width=\linewidth]{figures/network.pdf}
\caption{The structure of our network.}
\label{fig:network}
\end{center}
\end{figure}

Figure~\ref{fig:network} depicts our model for sentence generation
from videos. Our framework is based on recent deep image description
models in [cite LRCN, Oriol] and extending them to generate sentences
describing events in videos. These models work by first applying a
feature transformation on an image to generate a fixed dimensional
vector representation. They then use a sequence model, specifically a
Recurrent Neural Network (RNN), to ``decode'' the vector into a
sentence (i.e. a sequence of words). In this work, we apply the same
principle of ``translating'' a visual vector into an English sentence
and show that it works well for describing dynamic videos as well as
static images.

We identify the most likely description for a given video by training
a model to maximize the log likelihood of the sentence $S$,
given the coresponding video $V$ and the model parameters $\theta$,
$$ \theta^* = \argmax_{\theta} \text{ } \displaystyle\sum_{(V,S)} \text{log }p(S | V; \theta) $$

Assuming a generative model of $S$ that produces each word in the
sequence in order, the log probability of the sentence is given by
the sum of the log probabilities over the words and can be expressed
as:
$$ \text{ log } p(S | V) = \displaystyle\sum_{t=0}^{N} \text{log }p(S_{w_t} | V,
S_{w_1}, \ldots, S_{w_{t-1}} )$$
where $S_{w_i}$ represents the $i^{th}$ word in the sentence and N is the total
number of words. Note that we have dropped $\theta$ for convenience. 
%
%
%
%

A sequence model, such as an RNN is a natural choice to model $p(S_{w_t} | V,
S_{w_1}, \ldots, S_{w_{t-1}} )$. An RNN, parameterized by $\theta$,
maps an input $x_t$, and the previously seen words expressed as a hidden state
or memory, $h_{t-1}$ to an output $z_t$ and an updated state $h_t$ using a
non-linear function $f$:
$$h_t = f_{\theta}(x_t, h_{t-1})$$
where $(h_0 = 0)$. In our work we use the highly successful Long Short-Term Memory (LSTM) net as
the sequence model, since it has shown superior performance on tasks
such as speech recognition [cite Navdeep,Graves ICML], machine translation
[Yosua Bengio NIPS, GoogMT] and the more related task of generating
sentence descriptions of images [cite]. To be specific, we use two layers of
LSTMs (one LSTM stacked atop another) as shown in Figure 2 \vsub{Diagram of
unrolled LSTMs}. We present further details in Section \ref{subsec:lstm}.

To convert videos to a fixed length representation (input $x_t$), we
use a Convolutional Neural Network (CNN). [Side Note: This is one
  place where we differ from the LRCN paper's video description work.]
In particular, we use a hybrid of the publicly available
\textit{Caffe} \cite{caffe} reference model, a minor variant of the
\textit{AlexNet} \cite{alexnet}, and the network used by Zeiler and
Fergus \cite{ZF14eccv}. The net is pre-trained on the 1.2M image
ILSVRC-2012 object classification subset of the ImageNet dataset
\cite{imagenet} and hence provides a robust initialization for
recognizing objects and thereby expedites training. We present details
of how we apply the CNN model to videos in Section
\ref{subsec:vidrep}.

\subsection{LSTMs for sequence generation} \label{subsec:lstm}

A Recurrent Neural Network (RNN) is a generalization of feed forward neural
networks to sequences. Standard RNNs learn to map a sequence of inputs
($x_1,\ldots, x_t)$ to a sequence of hidden states ($h_1,\ldots, h_t)$, and from
the hidden states to a sequence of outputs ($z_1, \ldots, z_t$) based on the
following recurrences:
\begin{align*}
h_t &= f (W_{xh} x_t + W_{hh} h_{t-1}) \\
z_t &= g (W_{zh} h_t)
\end{align*}
where $f$ and $g$ are element-wise non-linear functions such as a
sigmoid or hyperbolic tangent, $x_t$ is a fixed length vector
representation of the input, $h_t \in \mathbb{R}^N$ is the hidden
state with $N$ units, $W_{ij}$ are the weights connecting the layers
of neurons, and $z_t$ the output vector.

RNNs can learn to map sequences for which the alignment between the
inputs and outputs is known ahead of time [Oriol MT] however it's
unclear if they can be applied to problems where the inputs ($x_i$)
and outputs ($z_i$) are of varying lengths. This problem is solved by
learning to map sequences of inputs to a fixed length vector using one
RNN, and then map the vector to an output sequence using another RNN.
Another known problem with RNNs is that, it can be difficult to train
them to learn long-range dependencies
\cite{hocreiter2001gradient}. However, LSTMs \cite{schmidLSTM}, which
incorporate explicitly controllable memory units, are known to be able
to learn long-range temporal dependecies and have been succesfully
applied to tasks such as machine translation \cite{GoogMT} and
sequence generation \cite{LRCN}.  In our work we use the LSTM unit
described in \cite{zaremba2014learning, LRCN} as shown in Figure
\ref{lstm_unit}.

\begin{figure}
\centering
            \includegraphics[width=0.5\textwidth]{figures/LSTM_unit.pdf}
    \caption{The LSTM unit replicated from \cite{LRCN} and other refs}
    \label{fig:lstm_unit}
\end{figure}

At the core of the LSTM model is a memory cell $c$ which encodes, at every time step,
the knowledge of the inputs that have been observed up to that step.
%
The cell is modulated by gates 
which are all sigmoidal, having range $[0,1]$ and are applied multiplicatively. 
The gates determine whether the LSTM keeps the value from the
gate (if the layer evaluates to 1) or discards it (if it evaluates to 0). The three gates --
input gate ($i$) controlling whether the LSTM considers it's current input ($x_t$),
the forget gate ($f$) allowing the LSTM to forget it's previous memory ($c_{t-1}$),
 and the output gate ($o$)
deciding how much of the memory to transfer to the hidden state ($h_t$), all enable the LSTM to learn
complex long-term dependencies. The recurrences for the LSTM are then 
defined as:
\begin{align*}
i_t &= \sigma(W_{xi} x_t + W_{hi} h_{t-1}) \\
f_t &= \sigma(W_{xf} x_t + W_{hf} h_{t-1}) \\
o_t &= \sigma(W_{xo} x_t + W_{ho} h_{t-1}) \\
c_t &=  f_t \odot c_{t-1}  + \phi(W_{xc} x_t + W_{hc} h_{t-1}) \\
h_t &= o_t \odot \phi(c_t)
\end{align*}
where $\sigma$ is the sigmoidal non-linearity, %
$\phi$ is the hyperbolic tangent non-linearity, and $\odot$ represents the product
with the gate value, and the weight matrices denoted by $W_{ij}$, the trained parameters. 

\subsection{LSTMs for video description}\label{subsec:vidrep}
The framework for our two layer LSTM model for generating descriptions
for videos is very similar to that used for generating image
descriptions in \cite{LRCN}. We employ the LSTM to ``decode" a visual
feature vector representing the video to generate textual output. The
first step in this process is to generate a fixed-length visual input
that effectively summarizes a short video. For this we use a CNN,
specifically a hybrid of the publicly available \textit{Caffe}
\cite{caffe} reference model. The net is pre-trained on the 1.2M image
ILSVRC-2012 classification subset of the ImageNet dataset. We extract
the output of the fc$_7$ layer for a set of sample frames in the video
(1 in every 10 frames) and perform a mean pooling over the frames to
generate a single 4,096 dimension vector for each video. The resulting
visual feature vector forms the input to the first LSTM layer. We
stack another LSTM layer on top as in Figure Main, and the hidden
state of the LSTM in the first layer is the input to the LSTM unit in
the second layer. A word from the sentence forms the target of the
output LSTM unit. In this work, we represent words using the
``one-hot" vector notation (i.e 1-of-N coding).

%
%
%

\paragraph{Training and Inference:}
The two-layer LSTM model is trained to predict the next word $S_{w_t}$ in the sentence
given the visual features and the previous $t-1$ words, $p(S_{w_t} | V,
S_{w_1}, \ldots, S_{w_{t-1}} )$. During training the visual feature,
sentence pair ($V,S$) is provided to the model, which then optimizes the
log-likelihood (refer equation) over the entire training dataset using
stochastic gradient descent. At each time step,
the visual feature vector
$x_t$ is input to the LSTM along with the previous time step's hidden state
$h_{t-1}$ and the LSTM emits the next hidden state vector $h_t$ (and a word).
Accordingly, inference must also be performed sequentially in the
order $h_1 = f_W(x_1, 0)$, $h_2 = f_W(x_2, h_1)$, until the model emits the stop word
at the final step $T$. In our model the output ($h_t$ = $z_t$) of the second
layer LSTM unit is used to obtain the emitted word. We apply the Softmax
function, to get a probability distribution over the words in the vocabulary. 
$$p_t(w_t) = \text{Softmax }(z_t) = \frac{\text{exp}(W_{zc}z_{t,c})}{\sum_{c' \in
C} \text{exp}(W_{zc}z_{t,c'})}$$
where $C$ in our case is the finite and discrete space determined by the vocabulary.
Thus, at each step we sample a word according to $p_t$ until we obtain the
end-of-sentence (EOS) token.

\subsection{Transfer Learning from Images}\label{subsec:transfer}
Since the training data available for video description is quite
limited (described in Section [ref data]) we also leverage much larger
datasets available for image description to train our LSTM model and
then fine tune this initial model on the video dataset. Our LSTM model
for images is the same as the one described above for single video
frames (in Section \ref{subsec:lstm}, and \ref{subsec:vidrep}). As
with videos, we extract \textit{AlexNet} fc$_7$ layer features (4096
dimensional vector) for the images. This forms the visual feature that
is input to the 2 layer LSTM description model. After the model is
trained on the image dataset, we use the weights of the trained model
to initialize the LSTM model for the video description
task. Additionally, we reduce the learning rate on our LSTM model to
allow for it to tune to the video dataset. This speeds up training
and allows exploiting knowledge previously learned for image description.
%
%

%




